Investigating Characteristics of Media Recommendation Solicitation in r/ifyoulikeblank

Despite the existence of search-based recommender systems like Google, Netflix, and Spotify, online users sometimes may turn to crowdsourced recommendations in places like the r/ifyoulikeblank subreddit. In this exploratory study, we probe why users go to r/ifyoulikeblank, how they look for recommendation, and how the subreddit users respond to recommendation requests. To answer, we collected sample posts from r/ifyoulikeblank and analyzed them using a qualitative approach. Our analysis reveals that users come to this subreddit for various reasons, such as exhausting popular search systems, not knowing what or how to search for an item, and thinking crowd have better knowledge than search systems. Examining users query and their description, we found novel information users provide during recommendation seeking using r/ifyoulikeblank. For example, sometimes they ask for artifacts recommendation based on the tools used to create them. Or, sometimes indicating a recommendation seeker's time constraints can help better suit recommendations to their needs. Finally, recommendation responses and interactions revealed patterns of how requesters and responders refine queries and recommendations. Our work informs future intelligent recommender systems design.

==> Original_tex/5result_backup.tex <==
\section{Results}
Below, we present the result of our analysis outlining the characteristics of queries, responses, and interactions developed through our coding process, along with a summary of our quantitative exploration of \sys{}.

% \sang{reviewed up to this point. }

\subsection{Characteristics of Queries and Responses}
Our coding process led to the development of a codebook with 10 codes and 37 sub-codes in total.
Table \ref{tab:rq1} shows the compiled codebook.
Out of these, 9 codes and 30 sub-codes relate to the characteristics of questions and answers, while the rest relate to interactions.
To contextualize characteristics that have been considered in recommender systems in the past, we looked for existing works using these characteristics in recommender system design papers and analyzed four search platforms (IMDB, Spotify, Steam, Amazon Books) to identify the available filters in their advanced search menus.
% Furthermore, we also used linguistic analysis to identify the number of occurrences of each subcode using a mixture of regular expressions and dictionary lists.
However, this analysis process is not perfect; it provides only a naïve representation.
We discuss these codes in detail below.

\begin{table}
    \centering
    \footnotesize
    \caption{Codes and sub-codes identified in qualitative open coding, answering our research question. Here, the Flair column shows the categories in which we encountered a given subcode. Some of these characteristics have been mentioned in prior literature. This reference list is not exhaustive. We checked four existing platforms for support for each sub-code as a filtering option. * indicates limited support.}
    \label{tab:rq1}
    \begin{tabular}{rlllcccc}
        & & & & \multicolumn{4}{c}{\textbf{Platform Supporting the Feature}}\\
        \cline{5-8}
        & & & & & & & \textbf{Amazon}\\
        \textbf{Code} & \textbf{Sub-code} & \textbf{Flair} & \textbf{Prior Refs.} & \textbf{IMDB} & \textbf{Spotify} & \textbf{Steam} & \textbf{Books}\\
        \midrule
         \multirow{9}{*}{Artifact}  &  Completeness  &  TV  & & NA & NA & NA & NA   \\
          &  Content  &  Games, Music  & \cite{Lyu2021, cremonesi2010, bountouridis2019} & \faicon{check} & \faicon{check} & \faicon{check} & \faicon{check}  \\ % Cuisine Type/Menu in a restaurant
          &  Date  &  Games, Music  & &  \faicon{check} & \faicon{check} & \faicon{check} & \faicon{check}\\
          &  Genre  &  Books, Film, Games, Music, TV  & \cite{Dias2014,Lyu2021, dhakad2017} & \faicon{check} & \faicon{check} & \faicon{check} & NA \\ % content feature to find weights, place with scenic view/Ambience/Noise level
          &  Language  &  Music, TV  & \cite{Seifert2015} & \faicon{check} & \faicon{check} & NA & \faicon{check}  \\ % for search results: preferred language of results
          &  Location  &  Film, TV  & \cite{Lyu2021, lu2016} & \faicon{check}* & NA & NA & NA  \\ % restaurant location
          &  Popularity  &  Music  & \cite{Lyu2021,Seifert2015, Sedhain2013} & \faicon{check} & \faicon{check} & \faicon{check} & \faicon{check} \\ % rating
          &  Revision  &  Music  & &  NA & NA & NA & NA \\
          &  Tools  &  Music  & &  NA & NA & NA & NA \\
        \hline
        \multirow{4}{*}{Artist}  &  Activity Level  &  Music  & & NA & NA & NA & NA  \\
          &  Demography  &  Music  & \cite{dai2014} & \faicon{check}* & NA & NA & NA \\
          &  Genre  &  Music  & & \faicon{check}* & \faicon{check}* & \faicon{check}*  & \faicon{check}* \\
          &  Popularity  &  Music  & &  \faicon{check}* & \faicon{check} & NA & \faicon{check}  \\
        \hline
        \multirow{2}{*}{Event}  &  Activity  &  Books, Film, Games, Music, TV  & \cite{Dias2014,Lyu2021,Zheng2016, mcinnis2016} & NA & \faicon{check} & \faicon{check} & NA \\ % activities were walking/relaxing/running/sleeping/shopping, enjoyable with family, family
          &  Scene  &  Games, Music  & \cite{Zheng2016} & NA & \faicon{check} & NA & NA\\ % time/day/season/location/weather
        \hline
        \multirow{1}{*}{Non-primary Entity}  &  *  &  Games, Music  & & \faicon{check}* & \faicon{check}* & \faicon{check}* & \faicon{check}*\\
        \hline
        \multirow{1}{*}{Platform}  &  *  &  Games, Music, TV  & & NA & NA & \faicon{check}* & \faicon{check}* \\
        \hline
        \multirow{5}{*}{Query}  &  Abbreviation  &  Film, Games, TV  & & \faicon{check} & \faicon{check} & \faicon{check} & \faicon{check}\\
          &  Adjectives  &  Music, TV  & & \faicon{check} & \faicon{check} & \faicon{check} & \faicon{check}\\
          &  Transcendence  &  Books, Games, TV  &  & NA & NA & NA & NA\\
          &  Image  &  Books, Music  & \cite{feldman2020} & NA & NA & NA & NA\\
          &  Justification  &  Games, Music  & \cite{Tsai2020,Lyu2021} & NA & NA & NA & NA\\ % users were asked to provide reason they choose an item, justify
          &  Specificity  &  Books, Games, Music, TV  & & NA & NA & NA & NA\\
        \hline
        \multirow{3}{*}{Response}  &  Justification  &  Film, Games, Music  & \cite{Cai2020,Lyu2021} & NA & NA & NA & NA\\
          &  Preview  &  Film  & \cite{jadidinejad2019} & NA & NA & NA & NA\\
          &  Transcendence  &  Music  & & NA & \faicon{check}* & NA & NA\\
        \hline
        \multirow{1}{*}{Recommender}  & Expertise  &  Music  & \cite{Lee2010,Lee2014} & NA & NA & NA & NA\\ % experts are those who listen to novice users recommendation in the short tail
        \hline
        \multirow{4}{*}{Recommendation Seeker} & Expertise/Acknowledgement  &  Games, Music  & \cite{Seifert2015} & NA & NA & NA & \faicon{check}*\\ % level of expertise in a information searching context, books have reader age
          &  Feeling  &  Games, Music  & \cite{Andjelkovic2019,Zheng2016} & NA & \faicon{check} & \faicon{check} & NA \\ % mood is tagged for the song by the artist, emotion
          &  Idiosyncrasy  &  Music  & & NA & NA & NA & NA \\
          &  Time Commitment  &  Film, Games  &  & NA & NA & NA & NA \\
          &  Willingness to Repeat  &  Film, Games  & & NA & NA & NA & NA\\
        \hline
        \hline\multirow{7}{*}{Interaction}  &  Affirming Taste  &  Music  & &  NA & NA & NA & NA \\
          & Discussion  &  Books  & \cite{Lyu2021} & NA & NA & NA & NA\\ % personal opinion, Comparison, Persuasion, Prior Experience
          & Endorsement  &  TV  & & NA & NA & NA & NA\\
          & Refinement  &  Books, Film, Games, Music, TV  & \cite{Cai2020,Lyu2021} & NA & NA & NA & NA\\
          & Repetition  &  Books, Games, Music  &  & NA & NA & NA & NA\\
          & Reciprocity  &  Music  & & NA & NA & NA & NA\\
        & Miscellaneous  &  Books, Film, Games, Music, TV  & \cite{Cai2020,Lyu2021,Seifert2015} & NA & NA & NA & NA\\ %,,recommendations desirable?
        \hline
    \end{tabular}
    % \vspace{-8pt}
\end{table}

\ssubsubsection{Artifact}
% The code ``Artifact'' describes the thing user is asking recommendation for, i.e., music/song, movie, tv series, books etc. Since this is the primary reason for posting on \sys{}, it is not surprising that a large number of codes (n) described the artifact. We found these description within the question, with a few in the answer and op's response. Within the artifact code, we found several subcodes describing various aspects of the artifact.
In this context, an Artifact is an object of the class within which a user is seeking recommendations, such as music/songs, movies, TV series, and books, among others. \sys{} rules ask users to mention up to nine Artifacts in post titles. We will look closer at their presence in our quantitative analysis. 
% Given the fundamental purpose of the posting here is seeking such artifacts, it is not surprising that we found nine subcodes used to describe the artifact. 
% These codes were identified within the question, with a few instances observed in the answer and the original poster's response. 
Within the Artifact code, nine sub-codes were employed to capture various facets of a given artifact. We discuss them here:

\noindent\textbf{Completeness.} Completeness indicates whether the creation or publication of an item is finished or ongoing. 
For instance, a user in our data set requested recommendations for complete TV series. 
Completeness could be described in various terms, including regarding a particular or final season. 
This category also applies to other artifacts, such as musical albums, movie series, book series, and so on. 
In some instances, we noticed that users preferred incomplete artifacts they could consume incrementally during the release period.
% Using linguistic analysis with regular expression matching, we found 67/19715 instances of this subcode being mentioned in our post sample.
None of the four platforms we checked support this feature as an option for filters or recommendation criteria.


\noindent\textbf{Content.}
% Content describes what the artifact consists of. 
% For example, content of a song is what the lyrics says or refers to or content of a movie is the story it describes. 
% When asking about content, OP did primarily seek certain things (e.g., biblical reference in a song) are there or whether any story exists inside (e.g., a series of albums tells a complete story).
% In games, OP asked for content with certain musics, dialogs, and stories.
% Though our dataset only referred to content for music and games, this subcode can also be extended to rest of of the artifacts.
Content refers to the substance of an artifact, which encompasses various elements central to its creation and interpretation. For example, the content of a song includes the lyrics and the themes that it expresses or refers to, while the content of a movie is the story that it tells, along with its characters, settings, and messages. Users seek specific details or elements that can help them better understand and appreciate an artifact when inquiring about content. In our data set, original posters (OP) sought content, such as biblical references in a song or the presence of a coherent story throughout a series of albums.

In the case of games, content includes such elements as musical scores, dialogues, and storylines which contribute to the overall gameplay experience. For example, ``looking for horror themed stories about private investigation'' appeared in a post in which the OP sought content that encompassed specific types of musical score, dialogue, and storyline to enhance their gaming experience. It is worth noting that while we found this subcode within content types of music and games, the subcode can also apply to other types of artifacts. 
Furthermore, users could be open to recommendations for multiple types of artifacts sharing such content attributes.
% With regular expression, we found 557/19715 instances of this subcode (e.g., ``old folk song in the story'' and ``looking for horror themed stories about private investigation'').
This is one of the common filters available across all the search systems we examined.
However, availability does not necessarily mean the recommendations from these systems match users' expectations.


\noindent\textbf{Date.}
OPs and responders both mentioned Artifacts coming from certain time periods.
We found OPs mentioning specific date ranges or names in titles and posts to clarify their requests.
Examples of such requests include music from a specific time frame (2011-2017), TV series with content depicting a certain kind of period (``futuristic dystopia''), and game backgrounds from certain times (``middle Ages'' and ``the 50s'').
Some of these items may intersect with Genre subcode. 
% Using Spacy Entity detection, we found 626/19715 mention of time among the posts.
All four recommender systems from our list already support searching artifacts by these characteristics, either in metadata through filters or keyword searches.


\noindent\textbf{Genre.}
A large number of observations were related to the genre of an artifact.
This code varied by content category.
In the context of music, OPs requested temporal characteristics (tempo, length of a song), atmospheric and storytelling qualities (triumph, epic, confident), and musical genres (fusing multiple genres).
In the context of games, they requested artifacts with a specific perspective for the main character (first vs. third person).
In the context of books, OPs requested protagonist or other character attributes (LGBT, outstandingly smart), high-level theme (fantasy), and meta-characteristics (stories about stories).
For TV and Film, OPs requested storytelling styles (non-linearity), dressing styles (costume, cool outfit, cowboy, leather), and high-level theme (mind-bending, psychological, rom-com).
% We found 5943/19715 reference to style in our dataset.
Generally, existing recommender systems allow artifact searches using this characteristic, and some unsolicited recommenders (e.g., Netflix home) often use this characteristic (e.g., rom-com) to categorize their recommendations.

\noindent\textbf{Language.}
In the TV Series and Music categories, OPs commonly asked for artifacts in a certain language.
These searches included asking for translated versions of artifacts in other languages, such as with subtitles or voice-over translation.
For example, an English-speaking user might be happy to be recommended anime in Japanese as long as English subtitles are available.
In other instances, such as a documentary or reaction video, the OP may instead request commentary or narration in a particular language.
Similar to other sub-codes, this one is also extensible to many types of artifacts, such as movies.
% For example, someone might be interested in movies in a certain language.
% We found 742/19715 mentions of languages in our dataset.
Among the four recommender systems we checked, only IMDB, Spotify, and Amazon Books allow filtering by language.

\noindent\textbf{Location.}
Location was a requirement for some OPs, who sought artifacts with geographic requirements at different levels. 
For example, OPs included region-level requirements (shows that take the time to incorporate elements of a given town or city) or landscape-level requirements (``movies that take place in the rainforest'').
We found that some posters specified examples to clarify their needs (e.g., ``I’m not searching genre-based, instead I’m searching for shows that make me feel like I’m living in those places. Californication in Cali, Justified [in] Kentucky, The Americans [in] DC'').
One OP mentioned that the rationale for this requirement was that they wanted artifacts that made them feel like they were in a certain place.
% In our post set, we found 457/19715 instances of location using SpaCy entity detection method.
Since this relates more to movies or tv series, IMDB seems to allow this filtering.
However, their filtering is cruder than the examples we mentioned here.

% \begin{quote}
%     Example: IIL movies that take place in the rainforest WEWIL? Bonus points for Tepuis, but by no means obligatory
% \end{quote}

\noindent\textbf{Popularity.}
For music, we found some OPs were interested in items with \textit{less} popularity.
One reason behind this requirement could be that they wanted to explore more music that they had not experienced before. 
While more popular artifacts are easily discoverable using online recommender platforms, the same cannot be said for less popular artifacts.
% Conducting regular expression check, we found 1287/19715 instances of mention of popularity.
However, this number includes the popularity of both artifacts and artists.

\noindent\textbf{Revision.}
Primarily in the context of music, some recommendation seekers sought out artifacts that were revisions of original artifacts.
These revisions had several typologies, such as remixes, covers, and even stylistic similarity.
Sometimes, an OP would ask for new content in the style of older content (e.g., ``a modern band creating music like Nirvana'').
Outside of music, this code could apply to adaptations of books into movies or TV shows.
% We looked keywords related to this characteristics and found 191/19715 matches.
Although these characteristics are not supported as a filter on the platforms we checked, some cues in artifact titles indicating revision status (e.g., ``cover by'', ``[remix]'') can be discovered in regular keyword searches. 



% \qt{OP}{I'm looking for a good anime with LGBT protagonists, queer themed or at least with significant queer storylines.}



\noindent\textbf{Tools.}
Sometimes, OPs requested artifacts created using specific tools.
For instance, in music, OPs asked for music featuring particular instruments, such as guitar, piano, and violin.
For TV and Films, they requested particular cinematography tools.
They also asked for certain combinations of instruments.
% Using a list of dictionary of musical tools\footnote{\url{https://github.com/imsky/wordlists/blob/master/nouns/music_instruments.txt}}, we found 1575/19715 matches to this characteristic in our dataset.
Among the four search platforms, none support filtering by this characteristic.

\ssubsubsection{Artist}
Besides Artifacts, we found many queries either described or asked for Artists---the primary creators of artifacts. We separated supporting production agents into a separate category. Although posters asked for Artists only in the context of music, the sub-code could apply to other categories, such as Movies. For Artists, we found four sub-codes: Artists' demography, theme of work, popularity, and activity level.
Below, we elaborate on them.

\noindent\textbf{Activity Level.}
For music, several data points indicated that OPs were interested in artists who were active creators at the time.
These activities were related to aspects such as music production and whether they were on tour (e.g., ``I’m trying to find similar stuff [to the band The Clash, specified in the title] by newer bands that are still making music and possibly touring. Ideas?''
This attribute is not supported as a filter in our platform set.
%, while the next subcode, i.e., demography could act as a supplement for this subcode to a certain extent. 

\noindent\textbf{Demography.} 
In several posts, OPs provided Artists' demographic backgrounds as criteria. Background information specified included artists' ethnicities (people of color), races (Black or White), individual or group gender identities (e.g., ``I m looking for something with screamy female vocal''), and relationships between artists within a group (e.g., siblings).
% Performing regular expression matching, we found 1003/19715 posts contained this subcode .
Among our list of platforms, IMDB has limited support for this, including searching by age and gender.

\noindent\textbf{Genre.}
Similar to the genre aspect under Artifact, several posts characterized an artist's genre as a requirement.
Such requirements included styling factors determined by the artist, such as the structure of content created, patterns of music (melancholic or slow-burn), popular categories (indie, Latin, jazz, rock), layering (building up various components), performance style of sections within a song (yelling or breaking down).
% Using regular expression, we found 1682/19715 mention of this characteristic in our post datset.
Within our set of platforms, we found limited support for this through keyword searches and genre filters.

\noindent\textbf{Popularity.}
In addition to activity level, some posters were interested in finding Artists that were less well-known or famous.
In one instance, OP asked for songs from less-known bands.
Therefore, this sub-code seems to be similar to its counterpart in Artifact.
With the exception of Steam, the other three platforms in our list seem to support this attribute as a filter or category (e.g., ``Hidden Gems'').


\begin{table}
    \centering
    \small
    \caption{Patterns. Punctuation marks and ``and'' separate items.}
    \label{tab:pattern}
    \begin{tabular}{p{0.45\linewidth}p{0.10\linewidth}p{0.40\linewidth}}
        \textbf{Pattern} & \textbf{\# Match} & \textbf{Matching Examples}\\
        \hline
        <song name> by <artist name> & 4721 & Click by Charlie, Blackstar by David Bowie, world.execute(me) by Mili \\
        these <song, artist, music> & 648 & these artists, this guy, These songs  \\
        <music, song, band> <like or about> <string> & 384 & artists like Girl Talk, Songs about suicide\\
        <song, music> that <verb> like <string> & 41 & song that sounds like it's the new single off your favorite band's best album \\
        \hline
        \multirow{5}{*}{Items matching no pattern} & \multirow{5}{*}{5648} & Rush E (Fanchen's rendition) as study music\\
        & & Genre and Record Label Compilation Albums\\
        & & Narrated music that tells a story\\
        & & Hip hop songs with beats like this?\\
        & & songs with dreamy instrumentals and fast lyrics\\
        \hline
    \end{tabular}
    % \vspace{-8pt}
\end{table}


\begin{table}
    \centering
    \small
    \caption{Strings to relevant item detection using google search }
    \label{tab:song_dist}
    \begin{tabular}{llll}
        \textbf{Type} & \textbf{\# among Matched Patterns} & \textbf{\# among Leftover} & \textbf{\# among All (unique)}\\
        \hline
         Artist & 203 & 1862 & 2065 (1292) \\
         Track & 1332 & 910 & 2242 (2029) \\
         Album & 149 & 223 & 372 (334) \\
         \hline
         All & & & 4679 \\
         % Tracks & & & 2029 \\
         \hline
    \end{tabular}
    
    % \vspace{-8pt}
\end{table}

% \sang{not sure if presenting quantitative result first is effective. }

\noindent\textit{Artists vs Artifacts: What do users mention more in post titles?}
With artists and artifacts being the primary object of interest, we examined how often users mention between these two in music.
Particularly, we looked for artists, tracks, and albums in post titles of 4183 posts which followed the formatting rules of the subreddit and received responses.
% since the rest of the data was harder to clean.
For this purpose, we first split strings on punctuation and ``and'', which resulted in 11442 strings.
Next, we manually examined the text and identified four patterns.
These patterns were: <song name> by <artist name>, these <song, artist, music>, <music, song, band> <like or about> <string>, <song, music> that <verb> like <string>.
For example, ``Blackstar by David Bowie'' matches the pattern <song name> by <artist name>.
We used the Spacy NLP toolkit~\footnote{\url{spacy.io}} to identify the strings that matched these patterns.
Table~\ref{tab:pattern} shows counts of these patterns with example matches, as well as examples of strings not belonging to any pattern.
After this, we used Google searches to identify whether the patterned strings referenced an artist, track, or album.
We used Google search because it enabled us to identify items better, even for strings not matching any pattern in the previous steps.
This process involved searching Google with each string and checking if the search results included a link to Spotify or Apple Music.
This process led to identification of 4679 artists, tracks, and albums.
Table~\ref{tab:song_dist} shows the resulting distribution.
Here, we found that artists and tracks were mentioned pretty evenly and held the majority, with relatively few (8\%) mentions of albums.
% We also noticed that 40\% of the artist references were duplicates.
Overall, artist and artifact mentions in titles indicate even interests by \sys{} users in each category.



\ssubsubsection{Event}
Event describes whether a particular artifact would be appropriate for use in a given setting. This code was used with all types of artifacts. The Event code consists of two subcodes, Scene and Activity, described below. 

\noindent\textbf{Activity.}
Some posters asked for artifacts to play during an activity.
Such activities included physical activities, such as workouts, dance and party,. Some wanted to create playlists for these activities.
Some also wanted to play (i.e., cover) particular songs themselves.
Typically, these requests also include targets the posters intend to involve: a multiplayer game to play with friends/family, a movie to watch with their significant other.
OPs may even mention the number of people involved (``4 player split screen game'').
% Sometimes, OPs would ask for content that could act as a memorabilia, for instance, for their dog.
Both Spotify and Steam support searching by this characteristic (e.g., ``workout music'').

\noindent\textbf{Scene.}
In several cases, OPs requested recommendations to play in various scenarios.
Such scene descriptions included locations (restaurants and cafes), other artifacts (songs or background music for a movie or commercial), abstract items (paintings), and environment (COVID isolation).
Using linguistic analysis, we found 3025/19,715 references to this attribute in our post set.
Among the four platforms, only Spotify has options for finding items by this attribute.

\ssubsubsection{Non-primary Production Entity}
Besides asking for recommendations based on an artifact or artist, there were a few instances where the OP asked for recommendations based on entities other than the primary artist involved in the production of an artifact. These requests included such entities as record labels for music, producers of movies, and the publisher of a game.
We did not identify any sub-codes under this code.
Among our four recommendation platforms, all of them provided some support for this feature as a filter.
For example, IMDB allows searching by company, and Spotify allows searching by label.

\ssubsubsection{Platform}
Since many artifacts are only available on certain online platforms, some posts also included a platform criterion.
For music, OPs might ask for songs available on Spotify.
For games, they might look for content playable on certain devices (mobile phone, PC, Xbox).
For TV shows, they might seek out content on Netflix (Netflix Originals) or YouTube.
This code also applies to regional availability, such as, Netflix India may have some content not available in Netflix USA.
% Our regular expression matcher identified 226/19715 matches to these keywords among the posts.
Among the four platforms, both Steam and Amazon Books provide partial sets of options to filter recommendation results by platform.
For example, Steam has filters for platform tags like Xbox, PC, Mac, and others.

\ssubsubsection{Query}
Examining the posts, we found that users formatted their posts in various ways.
We identified several characteristics here, including the use of abbreviations, adjectives, transcendence, images, justification, and specificity, described below. 

\noindent\textbf{Abbreviation.}
Posts sometimes used abbreviations for certain kinds of content.
Some of the abbreviations were ones that enjoy broad use (HIMYM for ``How I Met Your Mother'', DnD for ``Dungeons and Dragons'').
In some cases, posters created ad hoc abbreviations for their posts and reused them to refer to an item throughout the post text.
Abbreviations are generally recognized by the platforms in our list, although it can depend on how well-known the acronyms are. 


\noindent\textbf{Adjectives.}
In a few instances, OPs applied certain adjectives (surreal, mind-bending, cathartic) to a particular class of artifact.
These adjectives could sometimes be categorized as content genres (mind-bending), but not always (surreal, steamy).
Similar to abbreviations, genre-like adjectives are supported by recommender platforms in our list.


%\noindent\textbf{Generalization.}
\noindent\textbf{Transcendence.}
When seeking recommendations, OPs sometimes asked for recommendations that transcend multiple categories.
We termed this Transcendence (of the query scope).
For example, an OP might provide references in one category, like music, and ask for recommendations in other categories, like movies or TV shows (``lo-fi hip hop. Are there movies/TV shows that capture that vibe?'').
This characteristic is not supported by any platforms in our list.

% \qt{OP}{Video games, movies, shows, anything accepted but preferably (preferably) no books and podcasts (unless exceptionally good :-) ).}
% while being surrounded by advanced robotic animals. This new world has their own worries too, with these problems both big and small acting as the focus of both games.

\begin{figure}
    \centering
    \includegraphics[width=0.7\textwidth]{figures/322y00me3be91.jpg}
    \caption{Grid of images for an example query.}
    % \vspace{-8pt}
    \label{fig:grid_image}
\end{figure}

\noindent\textbf{Image.}
Some posters also made requests by posting sets of images of albums, songs, or books.
The purpose of formatting queries this way seemed to be to include particular art patterns not describable sufficiently through texts.
See Figure~\ref{fig:grid_image} for an example.
This input format is not supported by any platforms in our list.

\noindent\textbf{Justification.}
As part of their queries, OPs would sometimes provide justification for how they grouped items together.
This justification could be a short or long description (see the quote below).
Here, we see  a poster providing a long-winded description of a TV series episode and what they liked about it.
The four recommender systems in our list cannot currently account for this characteristic.
% however current progress in conversational recommender systems suggests that this is doable.

\qt{OP}{I really liked that episode and the way Bender gets to be a god, like him having his own prophet, his own commandments, the decision whether to answer to a prayer or not and seeing the consequences of his decisions, and seeing how his chosen people develop with their own free will. I have looked for games like these, but ...}
% they all look more like empires to me, or like sims. I don't wish to control the little people.

\noindent\textbf{Specificity.}
In several queries about different artifacts (music, games, and books), OPs provided different types of specific information in their queries.
These details were provided in terms of starting or ending time points (``0:32 second'', ``opening'', ``first 30 seconds'') for music and particular styles of writing within an author's works (``ending of under the dome by Stephen King'') for books.
Sometimes, these details were broad or nuanced (``Relaxing games that I can play with no stress'').
The four recommender systems in our list currently do not provide support for this feature.

\ssubsubsection{Response}
In our analysis, certain characteristics were prevalent in the recommendations provided by the commenters. We found three such characteristics, discussed below.

\noindent\textbf{Justification.}
When responding, commenters sometimes provided justification; that is, the reason they thought their recommendations matched the OP's criteria.
Sometimes, justifications were descriptive in nature; other times, they consisted of ratings, either from commenters themselves or from external reviewing sites.
Posters themselves sometimes responded to explain why a commenter's recommendation did not match their criteria.
See the examples of these interactions below.
Among our set of platforms, none provides justification. However, other platforms like Netflix provide limited justification (e.g., ``Because you liked [X]'').

% \qt{Recommender}{Bloodborne. Although, the Lovecraftian elements[OP's requirement] don't really show up until about halfway to two-thirds of the way through the game.}

\qt{Recommender}{Hollow Knight (Darkest game on this list, but easily the cutest and most beautiful. Give it time as the opening hours can sometimes put off new players. 10/10)}

% \qt{Recommender}{The Other Guys: \url{https://www.rottentomatoes.com/m/other_guys}}

\qt{OP}{Nightwish [a recommendation provided by the commenter], obviously talented vocalists (Tarja and Floor both), but symphonic power metal is not my cup of tea.}

\noindent\textbf{Preview.}
In some cases, commenters provided responses that included previews or snippets to entice the OP.
These previews could be taken from a trailer or certain section of an artifact (``The funeral scene [\url{https://www.youtube.com/watch?v=Oyj7YeXHhcA&ab_channel=Angie}] is amazing.'').
This feature is not supported by the platforms on our list.

\noindent\textbf{Transcendence.}
In their answers, recommenders sometimes provided content outside of the requested category, such as a game instead of a book (see quote below).
% Some would list out single items while others may lists such as playlists.
This is a counterpart to the similar characteristics under Query.
Among our list of platforms, Spotify provides a similarly generalized response through its search function, which can return matching tracks, playlists, albums, or artists.

\qt{Recommender}{[In response to book recommendation] Do stories from video games count? If so, the Horizon games, Zero Dawn and the just released Forbidden West, would interest you. The Earth of the past was destroyed, but humanity was preserved and started to rebuild ... }

 \ssubsubsection{Recommender}
From the recommender side, we found only one sub-code---expertise---which recurred in the responses.
For example, a recommender may not be familiar with all the items in a request while nonetheless having suggestions to offer.
The OP in one such instance was still receptive to the suggestions despite the knowledge gap.
This varying degree of expertise is not typically realized by current recommender systems, let alone by those on our list.

\qt{Recommender}{I actually haven't heard of any of the artists you've listed (I will have to check them out), but as for Canadian hip-hop artists, are you familiar with Cadence Weapon? I believe he won a Polaris prize a few years back.}

\ssubsubsection{Recommendation Seeker}
Sometimes, the requests revealed information about the OPs behind them despite the fact that none shared such information as a full activity history, demography, or other personality factors typically used by traditional recommender systems~\cite{Lu2018}.
We discuss these characteristics here.


\noindent\textbf{Expertise/Acknowledgement.}
In their queries, posters sometimes mentioned that they were uncertain about the ideal terms for what they were seeking. In such cases, they provided elaborate descriptions.
This strategy indicated that these users had a novice level of expertise.
Conversely, when OPs responded to comments, we noticed that some of them were receptive to trying lists of recommended items whenever they recognized at least a few items within the list (see quote below).
None of the platforms in our list are able to provide comparable information, indicating the extent of their knowledge in recommended results or specifying an expertise level. %; however, Amazon Books support a proxy feature through the ``Reader Age'' option.

\qt{OP}{[I] Like some King Tuff. Black Moon Spell is a banger. will definitely try out your other suggestions too.}

\noindent\textbf{Feeling.}
In the contexts of music and games, OPs mentioned their current state of mind as a way to find matching artifacts.
Such criteria included emotional states (sad, happy), vibes (getting over an ex, dark, drug addiction), or emotional responses to content consumption (eerie).
For example, one OP wrote ``I feel so safe whenever I watch these. They're so comforting.''
We have outlined the varying emotion and sentiment distributions of the posts in our list in our quantitative analysis section.
This characteristic is supported by three out of the four platforms in our list.
For example, Spotify allows listeners to find music by mood.
However, these options are likely limited to popular genres of music. 
% \sang{underwritten}

\begin{table}
    \centering
    \small
    \caption{Emotion and sentiment of posts.}
    \label{tab:emotion}
    \begin{tabular}{cc}
        \begin{tabular}{rlrlrl}
        \hline
        Joy          & 7903 & Sadness & 2136 & Surprise  & 29 \\
        Optimism     & 5359 & Disgust & 329  & Pessimism & 27 \\
        Anticipation & 3667 & Anger   & 308  & Trust     & 2  \\
        Love         & 2894 & Fear    & 287  &           &    \\ 
        \hline
        \end{tabular}
        &
        \begin{tabular}{rl}
            \hline
            Positive & 5071\\
            Neutral & 4752\\
            Negative & 519\\
            No majority & 9373\\
            \hline
        \end{tabular}
    \end{tabular}
    % \vspace{-8pt}
\end{table}


% \noindent\textit{Quantifying emotions and sentiments in \sys posts.}
To further contextualize this subcode, we quantitatively looked at emotions and sentiments present in all the posts (both title and body) using TweetNLP, a library primarily devised for tweets which also works well for short texts like Reddit posts~\cite{tweetnlp}.
Each of the models used in the classifiers was a fine-tuned version of roberta\footnote{\url{https://huggingface.co/cardiffnlp/twitter-roberta-base-2021-124m}} on TweetEval\footnote{\url{https://huggingface.co/datasets/tweet_eval}} tasks.
The result of this analysis is shown in Figure~\ref{tab:emotion}.
Note that the emotion classifier could assign multiple labels to a single post, so the sum can exceed the number of posts.
We found positive emotions such as Joy, Optimism, Anticipation, and Love ran high in the majority of the posts.
Still, 15\% of the posts showed negative emotions such as Sadness, Disgust, Anger, and Fear.
Looking into the emotional valence, we found that in half of the posts, no particular valence (positive, neutral, or negative) was dominant.
However, among the rest, a majority (95\%) were positive or neutral, with the remaining 5\% expressing negative sentiments.


\noindent\textbf{Idiosyncrasy.}
In rare cases, OP mentioned certain idiosyncrasies about who they are compared to what they like.
For example, one OP said, ``So I'm well aware my music taste is that of a 14-year-old TikTok obsessed, mentally ill Pinterest kid, and trust me I'm trying to get out of it.''
This sub-code could be covered by other characteristics for artifacts or artists.
However, we created this as a separate sub-code with a view towards capturing some of the nuances of the recommendation seekers.
This characteristic is not supported by the four platforms in our list.

\noindent\textbf{Time Commitment.}
One particular characteristic that affects recommendations is the availability of a user to consume the content.
Some requesters are able and willing to devote a large amount of time to consuming recommended content, such as playing a 100-hour game or binge-watching a 100-episode TV series.
Requesters expect to receive recommendations that fit these contraints.
The platforms on our list do not support this characteristic.
 
\noindent\textbf{Willingness to Repeat.}
Another characteristic that came up in several posts was whether posters would be open to repeating (rewatching or replaying) things they have consumed before.
In the words of one OP, ``Oh, maannnn!!! I haven't watched Ryan Trecarten's films in a while. I appreciate the reminder and the list.''
% Analyzing the data, we found 226/19715 matches about this openness to repeat.
Recommender systems can take this habit of recommendation seekers into consideration (e.g., Netflix's Watch it Again).

% To sum, these were the 9 high-level codes and underlying subcodes we found relevant to this research question.

\subsection{Characteristics of Interaction}

\begin{figure}
    \centering
    \includegraphics[width=0.75\textwidth]{figures/dist.pdf}
    % \vspace{-8pt}
    \caption{Distribution of user participation in \sys. (a) Y No. of user submitting X number of posts (b) Y No. of posts having X number of comments (c) Y No. of user submitting X number of comments. X axis is capped at 10. }
    \label{fig:dist}
\end{figure}

% \textit{How does user participation vary in \sys?}
For the interaction analysis, we first quantitatively looked at user participation in \sys.
Figure~\ref{fig:dist} shows user participation in \sys{}, showcasing the distribution of the posts and comments by users.
While this subreddit Figure~\ref{fig:dist}(a) shows that most posters (75\%) on \sys{} are one-time posters, with only 15\% posting twice.
Similarly to posters, a majority of commenters (57\%) on \sys{} are also one-time responders, with only 19\% commenting twice, as shown in Figure~\ref{fig:dist}(c).
Looking into comment count by posts that receive at least one comment, in Figure~\ref{fig:dist}(b), we found that 77\% of those posts received up to five comments.
Overall, we see that the interactions on this subreddit also look like a power law distribution with the long tail.


Next, our qualitative analysis of user interaction among the triplets revealed several sub-codes. 
These characteristics are not supported by the four platforms we examined.
However, these sub-codes could be incorporated inside conversational recommender systems to provide a better user experience. They can be applied to LLM-based conversational agents like ChatGPT or Google's Bard.
% We discuss them below.

\noindent\textbf{Affirming Taste}
In their interactions, commenters would sometimes respond just to express appreciation for OP's taste without offering a recommendation (e.g., ``great taste in music! just came to say that'').
In some cases, they would reveal that they had tastes similar to those of the OP (``We're like twins [with similar taste in music]'').
This type of interaction not only validates the OP's taste but also has the potential to create bonds between strangers on \sys.
Conversational recommender systems could promote a better human-like impression with this feature.

\noindent\textbf{Discussion.}
Sometimes, user interactions led to long conversations. 
We quantitatively identified long interaction chains.
We used heuristics of at least 3 back-and-forths; that is, chains of length 6.
This cutoff led us to identify 44 such conversations within our data set.
These discussions were not always between the OP and another commenter---some were between two or more other commenters.
These conversations fell into several themes.

\begin{itemize}
    \item Discussing a Particular Artist (4): Some conversations involved discussing a particular artist or band, their artifacts, and their evolution.
    \item Incremental Refinement of Recommendation (12): Some discussions between OP and a commenter revolved around incrementally refining suggestions as OP and the commenter went back and forth with restrictions. We further discuss refinement as a separate sub-code later.
    \item Sharing Playlists (2): When users realized they had similar tastes, they sometimes shared playlists with each other.
    \item Critiquing Item (Not) Matching (10): In many instances, two commenters discussed whether an item matched the criteria set by the OP.
    \item Discussing Requirement Homogeneity (4): Sometimes, commenters discussed whether items listed by the OP were homogenous, or whether the stated genre categorization made sense.
    \item Recommending Between Commenters (5): Some discussions led commenters to offer recommendations to each other.
\end{itemize}

\noindent\textbf{Endorsement.}
Among the interactions, in some instances, one commenter would endorse another's response with a comment (e.g., ``[In response to some other commenter's recommendation] Strongly seconding Alma's Not Normal and This Country - both are really great recs based on OP's list.'').
This does not necessarily add further information.
Although Reddit has upvotes and downvotes to operationalize endorsement, this behavior is still seen often.

\noindent\textbf{Refinement.}
As mentioned previously, we found 12 long interactions focused on refining recommendations.
Besides these, there were also shorter interactions where OP and commenters would try to refine criteria.
In some cases, the OP would provide exclusion criteria from the beginning (e.g., ``Nothing against death metal btw, just not what I'm looking for here.'')
OPs sometimes edited their posts to add criteria  (e.g., ``edit: similar vibe and love story stuff overall something not over corny like a notebook but not zero love and overall corniness little more or little less ...'').
Also, OPs could add criteria in response to a commenter's suggestion after identifying a mismatch (e.g., ``[in a comment] Although I really enjoy these tracks, it's not what I'm looking for exactly. It's tough to explain, it's the way the lead synth comes together with the bass which gives it a certain feel ...'').
In some instances, OPs mentioned that some of the suggestions from commenters were not available on their preferred platforms (e.g., ``she sounds great :) such a shame that I can't find her on Spotify'').
Sometimes, commenters sought clarification from OPs about vague or unclear requirements (e.g., ``What do you mean by `sometimes actively disliked' the institute?'').
% \qt{Commenter}{Do the suggestions need to have romance / a love story, or just similar vibes?}
OPs could also ask for clarification from commenters when recommendations were not specific enough---for instance, when there are multiple movies with the same name (e.g., ``Thanks! Also which year was The Guilty released? There's about 5 movies on IMDB with that name, and is the Carnage one the 2011 one?'').
To simulate these refinement interactions, a recommender system needs to hypothesize the gap first and implement some reasoning capacity.
% When commenters are not sure whether an item fits OP's requirement, they would express that in their comments.
% \qt{Commenter}{Majesty was[sic] somewhat close}

\noindent\textbf{Repetition.}
Sometimes, an OP would request the same recommendations over and over by posting a question repeatedly.
For example, one OP said, ``I'm sure I've asked similar questions to this in the past but I'm honestly always looking for more of this type of music''.
A recommender system needs to account for this type of interaction through memory and refine its responses appropriately.

\noindent\textbf{Reciprocity.}
When commenters responded by appreciating an OP's taste or indicating in any other way that they had similar tastes, the OP would sometimes provide some recommendation back to those commenters as a form of reciprocity.
This quote from an OP illustrates one such instance: ``Also, if you're interested, check out 'men in grey' by Hellfreaks. More hard rock than anything, but vocally you might like the vibe''.

% \qt{OP}{So far, we're up the same ally. Thank you for these suggestions. Takyon's great... have you heard the \href{https://soundcloud.com/annoyingringtone/annoying-ringtone-takyon-def-qon}{Annoying Ringtone dancecore flip} of it?}

\noindent\textbf{Miscellaneous.}
Many interactions between users fell into this category.
For instance, OPs responding with positive and negative responses fell into this category.
In some cases, these responses contained some elaboration, such as items OP liked or disliked.
% items they already knew, or items they didn't know.

To sum, these were the types of interactions we observed in \sys.
Current recommender systems can incorporate these characteristics to present better recommendations in the long-tail.
% , either through better modeling of the attributes inside the algorithm or through enabling customized filtration of the results.
We elaborate on the implications of these results in the Discussion section.



% \subsection{Characterizing \sys}
% Besides looking into the characteristics of long-tail recommendation seeking process, we also examined \sys{}.







% I will think about this
% \ssubsubsection{Topics Present}

% \begin{table}
%     \centering
%     \small
%     \begin{tabular}{rl}
%         \textbf{Topic ID} & \textbf{Keywords}\\
%         \hline
%         Topic -1 & drama, movies, fiction, tv, shows, books, character, media, characters, movie\\
%         Topic 0 & removed, deleted\\
%         Topic 1 & formatting, text, vsq, put, did, didnt, body, that, but, of\\
%         Topic 2 & kill, hurt, just, this, more, die, last, imagination, pure, so\\
%         Topic 3 & links, link, comments, comment, song, video, playlist, youtube, reference, in\\
%         Topic 4 & suggestions, thank, thanks, recommendation, appreciated, subreddit, subreddits, sub, mods, any\\
%         Topic 5 & songs, song, music, lyrics, genre, vocals, bands, album, albums, artists\\
%         Topic 6 & rpgs, games, gameplay, game, play, playing, fun, played, switch, experience\\
%         Topic 7 & youtube, videos, youtubers, channel, footage, movies, vhs, channels, streams, video\\
%         Topic 8 & podcast, podcasts, episodes, youtube, channel, documentary, intros, interviews, comedy, enjoyed\\
%         Topic 9 & anime, animes, cartoon, animation, protagonists, animated, shows, scififantasy, queer, nudity\\
%         Topic 10 & novels, books, book, reading, literary, recommendations, read, authors, themes, characters\\
%         Topic 11 & storylines, narratives, mythology, nonfictionthats, nonfiction, fiction, stories, manga, folklore, books\\
%         Topic 12 & movies, films, thrillers, thriller, film, movie, suggestions, watched, watching, horror\\
%         Topic 13 & shows, netflix, suggestions, tv, watching, seasons, movies, series, watch, favorite\\
%         Topic 14 & comedies, sitcoms, comedy, sitcom, comedic, humorescapism, shows, movies, humour, humor\\
%         \hline
%     \end{tabular}
%     \caption{Topic}
%     \label{tab:topic}
% \end{table}







\begin{figure}[t!]
    \centering
    \begin{subfigure}[t]{0.24\textwidth}
        \centering
        \includegraphics[width=0.95\textwidth]{figures/genre_1.pdf}
        \caption{All music genres from everynoise.com}
    \end{subfigure}%
    ~
    \begin{subfigure}[t]{0.24\textwidth}
        \centering
        \includegraphics[width=0.95\textwidth]{figures/genre_2.pdf}
        \caption{Genres of music mentioned in \sys{} posts}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.24\textwidth}
        \centering
        \includegraphics[width=0.95\textwidth]{figures/genre_3.pdf}
        \caption{Genres of music in four popular playlists on Spotify}
    \end{subfigure}
    \begin{subfigure}[t]{0.26\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figures/pair_plot.pdf}
        \caption{Pair plot of Spotify playlists and \sys ~genres}
    \end{subfigure}
    % \vspace{-8pt}
    \caption{Differences in presence of music genres.}
    \label{fig:genre-comp}
\end{figure}

\subsection{How diverse are \sys{} recommendations compared to popular recommendations? A Case Study of Music}
One of the premise of this study is that recommendation seekers come to \sys{} for recommendations in the long tail, i.e., the recommendation items they seek are not popular items.
We examined this premise by comparing music genre in the identified tracks (2242) in the post titles identified earlier against popular songs on Spotify.
The popular playlist songs were collected at the time of the analysis from the 30 most liked playlists on Spotify~\footnote{https://www.chosic.com/best-spotify-playlists/}, including Today's Top Hits, Pop Rising, Hot Hits USA, and New Music Friday.
There were 3728 tracks in this list, compared to the 2242 tracks in the \sys list.
To identify the genres, we used \url{everynoise.com} (mentioned in \sys), which listed 6049 music genres at the time of data collection.
Figure~\ref{fig:genre-comp} shows a comparison of song genres between all genres in everynoise.com, titles in 4183 posts in \sys{}, and the popular songs from Spotify.
Here, the X-Y coordinates of each genre are based on everynoise.com~\footnote{Everynoise.com suggests that ``the calibration is fuzzy, but in general down is more organic, up is more mechanical and electric [y-axis]; left is denser and more atmospheric, right is spikier and bouncier [x-axis].''}
Despite the popular Spotify playlists having more tracks, we found that the genres in \sys{} (781 unique) covered twice as many genres as the Spotify playlists (385 unique).
The average number of songs in each genre for \sys{} tracks (mean~=~2.19, SD~=~2.66) is lower than that of the popular Spotify playlists (mean~=~3.22, SD~=~5.64).
The distribution of song genres in \sys{} (mean~=~8874, SD~=~4680) along the X axis is closer to that of all genres (mean~=~10045, SD~=~5041) compared to that of popular Spotify playlists (mean~=~7453, SD~=~4338).
The distribution of song genres in \sys{} (mean~=~667, SD~=~273) along the Y axis is closer to that of all genres (mean~=~695, SD~=~309) compared to that of the popular Spotify playlists (mean~=~851, SD~=~250).
% It may also appear that \sys{} users have some bias towards the left half of the rectangle in this map.
In Figure~\ref{fig:genre-comp}(d), where the second row shows the projection of the Y axis, we see that Spotify playlists and \sys{} music genres have distribution peaks at opposing ends. 
% \sang{read my overleaf comment.}
To summarize, music genre in \sys{} is more diverse and different than popular songs on Spotify, with genre distribution being closer to all music genre.
This result signals that recommendation requests on \sys{} may indeed be about recommendations in the long tail.

